Generative Adversarial Imagination for Sample Efficient Deep Reinforcement Learning

Reinforcement learning has seen great advancements in the past five years. The successful introduction of deep learning in place of more traditional methods allowed reinforcement learning to scale to very complex domains achieving super-human performance in environments like the game of Go or numerous video games. Despite great successes in multiple domains, these new methods suffer from their own issues that make them often inapplicable to the real world problems. Extreme lack of data efficiency, together with huge variance and difficulty in enforcing safety constraints, is one of the three most prominent issues in the field. Usually, millions of data points sampled from the environment are necessary for these algorithms to converge to acceptable policies. This thesis proposes novel Generative Adversarial Imaginative Reinforcement Learning algorithm. It takes advantage of the recent introduction of highly effective generative adversarial models, and Markov property that underpins reinforcement learning setting, to model dynamics of the real environment within the internal imagination module. Rollouts from the imagination are then used to artificially simulate the real environment in a standard reinforcement learning process to avoid, often expensive and dangerous, trial and error in the real environment. Experimental results show that the proposed algorithm more economically utilises experience from the real environment than the current state-of-the-art Rainbow DQN algorithm, and thus makes an important step towards sample efficient deep reinforcement learning.

==> 1_header/glossary.tex <==
\newacronym{abc}{ABC}{Australian Broadcasting Corporation}

==> 3_appendices/submission.tex <==
The submitted zip file contains:
\begin{itemize}
    \item Figures used throughout the thesis (directory: \textbf{figures})
    \item Copy of the thesis (file: \textbf{kxk633\_kielak\_thesis.pdf})
    \item Sample research logs used for optimising hyperparameters (directory: \textbf{research\_logs})
    \item The Git repository address (file: git\_repository.txt)
    \item Source code (directory: \textbf{gairl})
\end{itemize}

The source code is structured as follows:
\begin{itemize}
    \item \textbf{requirements.txt} specifies required Python libraries.
    \item \textbf{resources} contains MNIST dataset used to debug and optimise generative models.
    \item \textbf{gairl} consists of the actual functional source code.
    \item \textbf{tests} includes unit tests for most critical and bug-prone parts of the code.
    \item \textbf{README.md} provides more detailed description of the code and how to successfully perform experiments.
\end{itemize}

Python3.6, together with libraries specified in the \textbf{requirements.txt} file, is a requirement. Additionally, Open AI Gym (included in the \textbf{requirements.txt}) may need \texttt{swig} and \texttt{python-opengl} packages (to install on Ubuntu\textgreater=16.04: \linebreak \texttt{sudo apt-get install -y swig python-opengl}). To properly run the code \texttt{PYTHONPATH} should point to the first level \textbf{gairl} directory.

Experiments can be executed by running one out of entry-points in the \linebreak \textbf{gairl/experiments} package. High-level configuration for the experiment can be set in the \textbf{gairl/config.py} file. Then, algorithm's (hyper)parameters can be changed in the appropriate algorithm-specific configuration file.

Additionally, the Git repository contains TensorBoard summaries of selected, previously performed experiments in its Git-LFS system (warning: they may take up to 7GB of space). Refer to the TensorBoard documentation on how to open the summaries. Moreover, commits history provides good overview of the implementation and experimentation progress (second term only, the first one was focused on reading and theoretical research).

